K-CONFIG: Using Failing Test Cases to Generate Test Cases in GCC Compilers

The correctness of compilers is instrumental in the safety and reliability of other software systems, as bugs in compilers can produce programs that do not reflect the intents of programmers. Compilers are complex software systems due to the complexity of optimization. GCC is an optimizing C compiler that has been used in building operating systems and many other system software. In this paper, we describe K-CONFIG, an approach that uses the bugs reported in the GCC repository to generate new test inputs. Our main insight is that the features appearing in the bug reports are likely to reappear in the future bugs, as the bugfixes can be incomplete or those features may be inherently challenging to implement hence more prone to errors. Our approach first clusters the failing test input extracted from the bug reports into clusters of similar test inputs. It then uses these clusters to create configurations for Csmith, the most popular test generator for C compilers. In our experiments on two versions of GCC, our approach could trigger up to 36 miscompilation failures, and 179 crashes, while Csmith with the default configuration did not trigger any failures. This work signifies the benefits of analyzing and using the reported bugs in the generation of new test inputs.

==> K-Means.tex <==
\section{\K{} Clustering}
\label{sec:kmeans}

The \K{} clustering is an unsupervised machine learning algorithm that performs clustering on unlabeled vector data. 
Given a set of vector data, this algorithm observes the underlying patterns and cluster similar data together. 
The number of clusters we want to see has to be predefined. 
Each cluster results in a centroid value that has a minimum distance to the data points of the cluster. 
The three key features which affect the result of \K{} are: (1) Distance Metrics, (2) Number of Clusters, and (3) Initial Setting for Clusters.



\subsection{Distance Metrics}
Suppose, $V$ is the vector data of $n$ observations and $k$ is the number of disjoint clusters $C$. The \K{} algorithm groups the $n$ observations into $k$ clusters and each cluster has a centroid $c$, the mean of the samples $V_c$ in the cluster. The centroid $c$ is set based on the minimum distance $d_m$ of inertia criterion. For \K{}, the distance metric is the within-cluster sum of squared distances which is defined as: 
\begin{align*}
  d_m = \sum_{i=0}^{n}\min_{c_i \in C, x_j \in V_{c_i}}(|c_i - x_j|^2)
\end{align*}

